A Novel Confidence-Based Algorithm for Structured Bandits

We study finite-armed stochastic bandits where the rewards of each arm might be correlated to those of other arms. We introduce a novel phased algorithm that exploits the given structure to build confidence sets over the parameters of the true bandit problem and rapidly discard all sub-optimal arms. In particular, unlike standard bandit algorithms with no structure, we show that the number of times a suboptimal arm is selected may actually be reduced thanks to the information collected by pulling other arms. Furthermore, we show that, in some structures, the regret of an anytime extension of our algorithm is uniformly bounded over time. For these constant-regret structures, we also derive a matching lower bound. Finally, we demonstrate numerically that our approach better exploits certain structures than existing methods.

==> sec_proof.tex <==
% !TEX root = main.tex

\section{Proof of Theorem \ref{th:regret-main}}\label{sec:proof}

{\color{red} We now prove the main regret bound of Theorem \ref{th:regret-main}. One of the key novelties and complications w.r.t. existing works is that, in order to carry out a fully structure-aware analysis, we do not only care about proving that sub-optimal arms are not pulled after certain phases, but also about guaranteeing that some arms are not discarded too early since their pulls might allow to discard other models/arms.} 

We begin by showing that, with high probability, the true model $\theta^*$ is always contained in the confidence set by a certain margin (which depends on $\beta$). Unlike previous works, we need this to guarantee that sub-optimal arms are not eliminated too early.

\begin{restatable}[]{lemma}{lemmaconf}\label{lemma:conf}
Let $\alpha >0$, $\beta \geq 1$, and $E = \{\forall h=0,\dots,\lceil \log_2 n \rceil : E_h\ \text{holds}\}$, with $E_h$ denoting the following event:
\begin{equation*}
E_h := \left\{ \forall i \in \mathcal{A} : |\hat{\mu}_{i,h-1} - \mu_i(\theta^*)| < \frac{1}{\beta} \sqrt{\frac{\alpha \log n}{T_i(h-1)}}\right\}.
\end{equation*}
Then, the probability that $E$ does not hold can be upper bounded by
\begin{equation*}
\prob{E^c} \leq |\mathcal{A}^*(\Theta)| n^{-2\frac{\alpha}{\beta^2}} (\log_2 n + 2)^2.
\end{equation*}
\end{restatable}
\mr{La notazione degli insiemi sopra non mi convince.}
We now show a condition on the number of pulls such that, under the 'good' event $E$, an arm is discarded.

\begin{restatable}[]{lemma}{lemmaarmel}\label{lemma:arm-el}
Let $h \geq 0$, $i \in \mathcal{A}$, and suppose that, for any model $\theta \in \Theta^*_i$ there exists an arm $j \in \mathcal{A}$  such that $T_j(h) \geq \left(1 + \frac{1}{\beta}\right)^2 \frac{\alpha \log n}{\Gamma_j^2(\theta, \theta^*)}$. Then, under event $E$, $i \notin \tilde{\mathcal{A}}_{h'}$ for all $h' > h$.
\end{restatable}

The following lemma states a condition on $\tilde{\Gamma}_{h-1}$ under which a model $\theta\neq\theta^*$ can be guaranteed to belong to $\tilde{\Theta}_h$.

\begin{restatable}[]{lemma}{lemmamodelinphase}\label{lemma:model-inphase}
Let $h \geq 1$, $\theta \in \Theta$, and $\alpha \geq \beta^2$. For all $i \in \mathcal{A}^*(\Theta)$, let $\tilde{h}_i \leq h - 1$ be such that either $i \notin \tilde{A}_{\tilde{h}_i + 1}$ or $\tilde{h}_i = h-1$. Suppose the following condition holds
\begin{align}\label{eq:cond-gamma}
    \tilde{\Gamma}_{h-1} \geq k_\beta \max_{j\in\mathcal{A}^*(\Theta)}\frac{\Gamma_j(\theta,\theta^*)}{2^{h - \tilde{h}_j - 1}}.
\end{align}
Then, under event $E$, $\theta \in \tilde{\Theta}_h$.
\end{restatable}

The following theorem is the key result that will be used to prove the final regret bound. It shows that the sets $\bar{\A}_h$ and $\underline{\A}_h$ defined in Section \ref{sec:sae} have the intended meaning.

\begin{restatable}[]{theorem}{tharmremoval}\label{th:arm-removal}
Let $\beta \geq 1$ and $\alpha = \beta^2$. Then, under event $E$, the following two statements are true for all $h \geq 0$:
\begin{align}\label{eq:armout}
&\forall i \in \bar{\mathcal{A}}_h : i \notin \tilde{\mathcal{A}}_{h'}\ \forall h'>h,\\
&\forall i \in \underline{\mathcal{A}}_h : i \in \tilde{\mathcal{A}}_{h}.\label{eq:armin}
\end{align}
\end{restatable}

\begin{proof}
We prove the theorem by induction on $h$.

\paragraph{1) Base case ($h = 0,1$)}

We show both $h=0$ and $h=1$ as base cases since the recursive definition of the sets $\underline{\mathcal{A}}_h$ starts from $h=1$ and depends on $\bar{\mathcal{A}}_h$. The recursive definition of the latter, on the other hand, starts from $h=0$.

\paragraph{1.1) First phase ($h=0$)}

Since $\tilde{A}_0 = \mathcal{A}^*(\Theta)$ by the initialization step of Algorithm \ref{alg:isucb}, \eqref{eq:armin} trivially holds. If $\bar{\mathcal{A}}_0$ is empty, \eqref{eq:armout} trivially holds as well. Suppose $\bar{\mathcal{A}}_0$ is not empty and fix any arm $i \in \bar{\mathcal{A}}_0$. For all arms $j \in \mathcal{A}^*(\Theta)$,
\begin{align*}
T_{j}(0) &\stackrel{(a)}{=} \left\lceil\frac{\alpha\log n}{\tilde{\Gamma}_{0}^2}\left(1 + \frac{1}{\beta}\right)^2\right\rceil
\\ &\stackrel{(b)}{\geq} \left\lceil\frac{\alpha\log n}{\inf_{\theta\in\Theta^*_i} \max_{l \in \mathcal{A}^*(\Theta)} \Gamma_l^2(\theta, \theta^*)}\left(1 + \frac{1}{\beta}\right)^2\right\rceil,
\end{align*}
where (a) is from the number of pulls in Algorithm \ref{alg:isucb} and the fact that all arms in $ \mathcal{A}^*(\Theta)$ are active, and (b) follows from the definition of $\bar{\mathcal{A}}_0$. Therefore, for all $\theta \in \Theta^*_i$ there exists some arm $j\in \mathcal{A}^*(\Theta)$ whose number of pulls at the end of phase $0$ is at least
\begin{align*}
    T_j(0) \geq \left\lceil\frac{\alpha\log n}{\Gamma_j^2(\theta, \theta^*)}\left(1 + \frac{1}{\beta}\right)^2\right\rceil.
\end{align*}
Hence, Lemma \ref{lemma:arm-el} ensures that $i \notin \tilde{\mathcal{A}}_{h'}$ for all $h'>0$, which in turn implies that \eqref{eq:armout} holds.

\paragraph{1.2) Second phase ($h=1$)}

Let us start from \eqref{eq:armin}. Take any arm $i \in \mathcal{A}_1 := \mathcal{A}^*(\Theta) \setminus \bar{\mathcal{A}}_0$ and suppose
\begin{align}\label{eq:lb-gamma}
    \tilde{\Gamma}_{0} > k_{\beta}\inf_{\theta\in\Theta^*_i} \max_{j \in \mathcal{A}^*(\Theta)} \frac{\Gamma_j(\theta, \theta^*)}{2^{\max\{-\bar{h}_j,0\}}}
\end{align}
holds. Since $2^{\max\{-\bar{h}_j,0\}} = 1$ for all $j \in \mathcal{A}^*(\Theta)$, \eqref{eq:lb-gamma} implies that there exists some model $\bar{\theta} \in \Theta^*_i$ such that $\tilde{\Gamma}_{0} \geq k_{\beta} \max_{j \in \mathcal{A}^*(\Theta)} \Gamma_j(\bar{\theta}, \theta^*)$.
 Thus, we can directly apply Lemma \ref{lemma:model-inphase} using $\tilde{h}_j = 0$ for all $j \in \mathcal{A}^*(\Theta)$ and obtain $\bar{\theta} \in \tilde{\Theta}_1$. This implies $i \in \tilde{\mathcal{A}}_1$, from which \eqref{eq:armin} holds.

The proof of \eqref{eq:armout} proceeds similarly as for $h=0$. Take any arm $i \in \bar{\mathcal{A}}_1$ (assuming the set is not empty). We have just proved that all arms $j \in \underline{\mathcal{A}}_1$ are pulled in phase $h=1$. If arm $i$ has already been removed, \eqref{eq:armout} trivially holds. Hence, we can safely assume that $i\in\tilde{\mathcal{A}}_1$. Therefore, arms in $\underline{\A}_1 \cup \{i\}$ are active and the number of pulls is sufficient to apply Lemma \ref{lemma:arm-el}, which implies \eqref{eq:armout}.

\paragraph{2) Inductive step ($h > 1$)}

Now assume the two statements hold for $h'=0,1,\dots,h-1$. This implies, in particular, that an arm $i\in\bar{\mathcal{A}}_{h'}$, $h'\leq h-1$, is not pulled after $h'$. Once again, take any arm $i \in \underline{A}_h$.
%\begin{align*}
%    \tilde{\Gamma}_{h-1} > k_{\beta,\gamma}\inf_{\theta\in\Theta^*_i} \max_{j \in \mathcal{A}^*(\Theta)} \frac{\Gamma_j(\theta, \theta^*)}{2^{\max\{h-\bar{h}_j-1,0\}}}
%\end{align*}
The definition of $\underline{A}_h$ implies
\begin{align*}
    \tilde{\Gamma}_{h-1} \geq k_{\beta}\max_{j \in \mathcal{A}^*(\Theta)} \frac{\Gamma_j(\bar{\theta}, \theta^*)}{2^{\max\{h-\bar{h}_j-1,0\}}}
\end{align*}
for some $\bar{\theta} \in \Theta^*_i$. Notice that, by the inductive assumption, all arms $j \in \mathcal{A}^*(\Theta) \setminus \mathcal{A}_h$ are not pulled after $\bar{h}_j \leq h-1$. On the other hand, for all arms $j \in \mathcal{A}_h$, it must be that $\bar{h}_j \geq h$. Thus, we can apply Lemma \ref{lemma:model-inphase} by setting $\tilde{h}_j = \bar{h}_j$ for arms $j \in \mathcal{A}^*(\Theta) \setminus \mathcal{A}_h$ and $\tilde{h}_j = h-1$ for arms $j \in \mathcal{A}_h$. Hence, $\bar{\theta} \in \tilde{\Theta}_h$ and \eqref{eq:armin} holds.

Finally, since all arms in $\underline{\mathcal{A}}_h$ are pulled in phase $h$, we can show that \eqref{eq:armout} holds using exactly the same argument as for the second base case ($h=1$).

\end{proof}

We are now ready to prove Theorem \ref{th:regret-main}.

\begin{proof}{\emph{(Theorem \ref{th:regret-main})}}
The expected regret can be written as
\begin{align*}
R_n &\stackrel{(a)}{\leq} \sum_{t=1}^n \expec{\Delta_{I_t}(\theta^*) | E} + n\prob{E^c}\\ &\stackrel{(b)}{=} \sum_{i \in \mathcal{A}} \Delta_i(\theta^*) \expec{T_i(n) | E} + n\prob{E^c},
\end{align*}
where in (a) we upper bounded the gaps by $1$ and used $\expec{\indi{E^c}} = \prob{E^C}$, while in (b) we used the standard rewriting in terms of the number of pulls.

We now upper bound the expected number of pulls of each sub-optimal arm $i$ when conditioned on event $E$. Since $i \in \bar{\mathcal{A}}_{\bar{h}_i}$, Theorem \ref{th:arm-removal} ensures that arm $i$ is not pulled after phase $\bar{h}_i$. Hence,
\begin{align*}
T_i(n) &\stackrel{(a)}{\leq} \left\lceil\frac{\alpha\log n}{\tilde{\Gamma}_{\bar{h}_i}^2}\left(1 + \frac{1}{\beta}\right)^2\right\rceil \stackrel{(b)}{=} \left\lceil\frac{4\alpha\log n}{\tilde{\Gamma}_{\bar{h}_i - 1}^2}\left(1 + \frac{1}{\beta}\right)^2\right\rceil\\ &\stackrel{(c)}{\leq} \left\lceil\frac{4(1+\beta^2)\log n}{\inf_{\theta\in\Theta^*_i} \max_{j \in \A_i^*} \Gamma_j^2(\theta, \theta^*)}\right\rceil,
\end{align*}
where (a) follows immediately from Theorem \ref{th:arm-removal} and Algorithm \ref{alg:isucb}, while (b) from $\tilde{\Gamma}_{\bar{h}_i} = \frac{\tilde{\Gamma}_{\bar{h}_i-1}}{2}$. To show (c), notice that $\tilde{\Gamma}_{\bar{h}_i - 1} > \inf_{\theta\in\Theta^*_i} \max_{j \in \A_i^*} \Gamma_j(\theta, \theta^*)$ from the definition of $\bar{\mathcal{A}}_{\bar{h}_i}$ (if this did not hold, arm $i$ would be eliminated in phase $\bar{h}_i-1$ since $\underline{\mathcal{A}}_{\bar{h}_i} \subseteq \underline{\mathcal{A}}_{\bar{h}_i-1}$). Therefore, the regret conditioned on event $E$ can be upper bound by
\begin{align*}
\sum_{i \in \mathcal{A}^*(\Theta)} \frac{4(1+\beta^2)\Delta_i(\theta^*)\log n}{\inf_{\theta\in\Theta^*_i} \max_{j \in \A_i^*} \Gamma_j^2(\theta, \theta^*)} + |\mathcal{A}^*(\Theta)|,
\end{align*}
where we used $\lceil x \rceil \leq x + 1$ and $\sum_{i \in \mathcal{A}^*(\Theta)} \Delta_{i}(\theta^*) \leq |\mathcal{A}^*(\Theta)|$.

Let us now consider the probability of $E$ not holding. Using Lemma \ref{lemma:conf} with $\alpha = \beta^2$, together with $(\log_2 n + 2)^2 \leq n$ for $n\geq 64$, we obtain
\begin{align*}
n\prob{E^c} \leq |\mathcal{A}^*(\Theta)|\frac{(\log_2 n + 2)^2}{n} \leq |\mathcal{A}^*(\Theta)|,
\end{align*}
which, combined with the previous bound, concludes the proof.

\end{proof}

==> table.tex <==
\begin{table*}[t!]
\centering
\begin{small}
\begin{tabular}{@{}lccccc@{}} 
\toprule
Structure & Lower Bound & UCB & SUCB & SAE & OSSB \\
\cmidrule{1-6}
Unstructured & $\mathcal{O}\left(\sum_i \frac{\log n}{\Delta_i(\theta^*)}\right)$ & Finite-time & Finite-time & Finite-time & {\color{red} Finite-time (?)} \\
Hard & $\mathcal{O}\left(\sum_i \frac{\Delta_i(\theta^*)\log n}{\inf_{\theta\in\Theta_i^+}\Gamma_i^2(\theta,\theta^*)}\right)$ & \ding{55} & Finite-time & Finite-time* & {\color{red} Finite-time (?)} \\
Constant-regret (hard) & $\mathcal{O}\left(\sum_i \frac{\Delta_i(\theta^*)\log (1/\Gamma_*)}{\inf_{\theta\in\Theta_i^*}\Gamma_i^2(\theta,\theta^*)}\right)$ & \ding{55} & Finite-time & Finite-time & N/A \\
General (confusing) & Optimization problem & \ding{55} & \ding{55} & \ding{55} & Asymptotic \\
\addlinespace[0.1cm]
General (no confusing) & \textbf{?} & \ding{55} & \ding{55} & \ding{55} & N/A  \\
\bottomrule
\end{tabular}
\end{small}
\caption{\emph{Order-optimality} (finite-time, asymptotic, or none) in different structures. \emph{Hard} structures are those that admit instances that are indistinguishable from the true model except for one arm. \emph{Constant-regret (hard)} structures (Section \ref{sec:lb}) are equivalent to hard structures where Assumption \ref{ass:dist} holds for a sufficiently small $\Gamma_*$. \emph{General (confusing)} structures are those considered by \cite{combes2017minimal}, while \emph{general (no confusing)} are those where no confusing model exists. *: optimal under the condition of Proposition \ref{prop:comparison-SUCB}. \todoal{Forse mettere i bound direttamente nella tabella e in ogni caso le strutture vanno definite da qualche parte in modo formale.}\todoa{Questa cerco di sistemarla alla fine. Ora le strutture worst-case e worst-case constant-regret sono introdotte. Devo trovare come e dove introdurre le altre due}}
\label{tab:algs}
\end{table*}

